Off-Policy Evaluation of Slate Bandit Policies via Optimizing Abstraction

We study off-policy evaluation (OPE) in the problem of slate contextual bandits where a policy selects multi-dimensional actions known as slates. This problem is widespread in recommender systems, search engines, marketing, to medical applications, however, the typical Inverse Propensity Scoring (IPS) estimator suffers from substantial variance due to large action spaces, making effective OPE a significant challenge. The PseudoInverse (PI) estimator has been introduced to mitigate the variance issue by assuming linearity in the reward function, but this can result in significant bias as this assumption is hard-to-verify from observed data and is often substantially violated. To address the limitations of previous estimators, we develop a novel estimator for OPE of slate bandits, called Latent IPS (LIPS), which defines importance weights in a low-dimensional slate abstraction space where we optimize slate abstractions to minimize the bias and variance of LIPS in a data-driven way. By doing so, LIPS can substantially reduce the variance of IPS without imposing restrictive assumptions on the reward function structure like linearity. Through empirical evaluation, we demonstrate that LIPS substantially outperforms existing estimators, particularly in scenarios with non-linear rewards and large slate spaces.

==> results/app_result_various.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.99\hsize}
\centering
\scalebox{0.95}{
\begin{tabular}{c}
\begin{minipage}{0.80\hsize}
\begin{center}
\includegraphics[width=1.025\linewidth]{figs/label.png}
\vspace{-2mm}
\end{center}
\end{minipage}
\\
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=1.02\linewidth]{figs/app/slate_size_delicious_.png}
        \vspace{-2mm}
        \caption{Comparison of the estimators' MSE (normalized by the true value $V(\pi)$) with varying slate sizes ($L$), reward functions (1) - (3), and randomly sampled configurations on Delicious.}
        \label{fig:slate_size_delicious_app}
        \vspace{3mm}
    \end{center}
\end{minipage}
\\
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=1.02\linewidth]{figs/app/slate_size_eurlex_.png}
        \vspace{-2mm}
        \caption{Comparison of the estimators' MSE (normalized by the true value $V(\pi)$) with varying slate sizes ($L$), reward functions (1) - (3), and randomly sampled configurations on Eurlex-4K.}
        \label{fig:slate_size_eurlex_app}
        \vspace{3mm}
    \end{center}
\end{minipage}
\\
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=1.02\linewidth]{figs/app/slate_size_wiki_.png}
        \vspace{-2mm}
        \caption{Comparison of the estimators' MSE (normalized by the true value $V(\pi)$) with varying slate sizes ($L$), reward functions (1) - (3), and randomly sampled configurations on Wiki10-31K.}
        \label{fig:slate_size_wiki_app}
        \vspace{3mm}
    \end{center}
\end{minipage}
\\ 
\\
\end{tabular}
}
\end{minipage}
\end{figure*}

==> results/main_result_2.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[clip, width=1.00\linewidth]{figs/delicious/data_size_delicious_additive.png}
    \vspace{-7mm}
    \caption{Estimators' performance comparison with various reward functions}
    \label{fig:delicious_variaous_reward_function}
\end{figure}

==> results/main_result_3.tex <==
\begin{figure*}[t]
\begin{minipage}[c]{0.99\hsize}
\centering
\scalebox{0.95}{
\begin{tabular}{c}
\begin{minipage}{0.55\hsize}
\begin{center}
\includegraphics[width=1.0\linewidth]{figs/label.png}
\end{center}
\end{minipage}
\\
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=1.0\linewidth]{figs/eurlex/lips_4_eurlex_additive.png}
        \vspace{-7mm}
        \caption{LIPS' performance comparison with varying choice of $\beta$ ($L=4$)}
        \label{fig:delicious_beta_6}
        \vspace{3mm}
    \end{center}
\end{minipage}
\\ 
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \includegraphics[clip, width=1.0\linewidth]{figs/eurlex/lips_8_eurlex_additive.png}
        \vspace{-7mm}
        \caption{LIPS' performance comparison with varying choice of $\beta$ ($L=8$)}
        \label{fig:delicious_beta_8}
        \vspace{3mm}
    \end{center}
\end{minipage}
\\
\\
\begin{minipage}{0.99\hsize}
    \begin{center}
        \begin{minipage}{0.35\hsize}
        \begin{center}
            \includegraphics[clip, width=1.0\linewidth]{figs/eurlex/heatmap_4_eurlex_additive.png}
        \end{center}
        \end{minipage}
        \begin{minipage}{0.35\hsize}
        \begin{center}
            \includegraphics[clip, width=1.0\linewidth]{figs/eurlex/heatmap_8_eurlex_additive.png}
        \end{center}
        \end{minipage}
        \vspace{0mm}
        \caption{Hyperparameter selection results of SLOPE; (Left) $L=4$; (Right) $L=8$}
        \label{fig:delicious_beta_12}
        \vspace{3mm}
    \end{center}
\end{minipage}
\\
\\
\end{tabular}
}
\end{minipage}
\end{figure*}
